The Rise of AI-Generated Content in Wikipedia

The rise of AI-generated content in popular information sources raises significant concerns about accountability, accuracy, and bias amplification. Beyond directly impacting consumers, the widespread presence of this content poses questions for the long-term viability of training language models on vast internet sweeps. We use GPTZero, a proprietary AI detector, and Binoculars, an open-source alternative, to establish lower bounds on the presence of AI-generated content in recently created Wikipedia pages. Both detectors reveal a marked increase in AI-generated content in recent pages compared to those from before the release of GPT-3.5. With thresholds calibrated to achieve a 1% false positive rate on pre-GPT-3.5 articles, detectors flag over 5% of newly created English Wikipedia articles as AI-generated, with lower percentages for German, French, and Italian articles. Flagged Wikipedia articles are typically of lower quality and are often self-promotional or partial towards a specific viewpoint on controversial topics.

==> sections/05_modification.tex <==
\section{Expanding the Scope with Updated Data}
\label{sec:more}

%past student essays.  \citet{wang-etal-2024-m4} aggregate Wikipedia, Wikihow, Reddit, arXiv, and PeerRead for their English sources.  However, most of this content such as the Wikipedia corpus is from before 2022, which makes  GenAI detection moot.  

Given that AI detection is still an art as much as a science, and depends on training data, we also investigate Reddit posts, news articles, and press releases.

%Specifically, we collect a corpus of new Wikipedia pages \textit{released in the last month}, which totals 6,705.
%
We focus Reddit analysis on contentious subreddit topics provided daily through Kaggle---Israel-Palestine, public opinion on Democrats, public opinion on Republicans---extended into 2024.  This consists of  4,747 posts.\footnote{Since GPTZero charges by the word, we sample 3,000 items from Wikipedia and Reddit that >=100 words in length.}

We follow \citet{verma2023ghostbuster} and \citet{hans2024spotting} in using AI detection on the news.  Rather than rely on the Reuters corpus by ~\citet{Houvardas2006NGramFS}, we collected a new pool of recent news stories as follows.
%
To avoid scraping concerns, we manually collected 50 stories comprised of articles on each of five topics (U.S., World, Business, Entertainment, Opinion if applicable) from each of the top 10 news sources  according to online traffic (NYTimes, CNN, FoxNews, People, USAToday, NYPost, DailyMail, WashingtonPost, BBC, and CNBC according to Statista (Figure~\ref{fig:statista}).

Unfortunately, these sources have stricted licensing so we cannot redistribute the data.  

\begin{comment}
\section{Bypassing Detection}
\label{sec:mod}

Currently there are few incentives to avoid detection as AI generated.  This will  change.

Watermarking has been developed to identify content generated by AI.  Copyright lawsuits have prompted tech companies to pursue content parternships with media sources.  

Based on past work and our own explorations, we provide an initial set of robustness checks for determining whether a given population is likely to contain AI-generated content: comparisons of detection rates in sources pre- and post-2023, 

\ai{this kinda comes out of nowhere:} the length of the content, and whether content generated by AI to be similar to content from the same distribution is readily detectable. We find that many AI detectors fail these robustness checks in common forms of data, including Binoculars and GhostBuster, especially for short-form content (\textbf{NEED TO DO OR SCRAP}). 

While caution is required for drawing conclusions at the individual level, focusing these methods on large distributions of content can be used to estimate trends and problem areas.

\ai{Not sure what the intended implication is here or why it's here rather than 5.1?}
A Wikipedia article that skims just below the .5 threshold of GPTZero about Rexhep Ferri escalates to a .98 score when the Albanian language publications, which comprise the second half of the article, are removed.  
\begin{figure}[H]
  \includegraphics[width=\linewidth]{figures/wiki2.png} 
\end{figure}    

\end{comment}

==> sections/UNSection.tex <==

\section{A New Domain: Press Releases from United Nations Country Teams}
\label{sec:un}

Here we raise the critical question as to whether prior results apply to a new domain. 
In particular, we investigate press releases from a well-known organization, the country teams of the United Nations. We collect 8326 press releases across 60 countries from 2013 to 2024 and use a subset to test and compare the AI detection models (Section~\ref{sec:comp}).

The United Nations "remains the one place on Earth where all the world’s nations can gather together, discuss common problems, and find shared solutions that benefit all of humanity".\footnote{\url{https://www.un.org/}}  Country teams of the United Nations provide frequent updates about developments in that country.
%
\begin{comment}
\begin{figure*}[t]
  \includegraphics[width=.9\linewidth]{figures/bangladesh.png} 
  \includegraphics[width=.9\linewidth]{figures/bangladesh_binoculars.png} 
\caption {Releases by the UN about Bangladesh have have a notable uptick in content detected as AI by \texttt{GPTZero} (top panel), while \texttt{Binoculars} sucks \textbf{...XXXXX} (bottom panel)\textbf{Need to align the x axes so we're looking at apples and apples here; reverse axes on bottom panel if up fails to mean more detection }
  Temp Figures, Actual Data}
  
\end{figure*}
\end{comment}
%
Such data is an important domain to study for several reasons. Unlike Reddit or Wikipedia, the majority of UN press releases identify their authors---with names rather than aliases---who are often UN senior officials and affiliates.
%
Like the news, press releases are topical and focus on detailed issues. 
%
However, unlike the news, the content of press releases is optionally and non-commercially published to disseminate respective countries' accomplishments in the context of the United Nations.  For our data collection, we scrape all press releases that are made by country teams that have websites in the format of \url{https://{country}.un.org}. For example, \url{https://georgia.un.org}.

\begin{table}[h!]
    \small
    \centering
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Model} & \textbf{AUROC} & \textbf{Precision} & \textbf{Recall} & $\mathbf{F_{1}}$ \\
        \midrule
        GPTZero &    0.98 & 1.0  & 0.51 & 0.68 \\
        Binoculars  & 0.81 & 1.0  & 0.42 & 0.59 \\
        Ghostbuster & 0.85 & 0.71 & 1.0  & 0.83 \\
        \bottomrule
    \end{tabular}
    \caption{Performance metrics for different models. A precision of 1.0 indicates that the model did not misclassify any human text as AI-generated, and a recall of 1.0 indicates that all text with AI-generated content was classified as such. Since these metrics rely on a threshold, we consider AUROC is the most useful metric; altering \texttt{GPTZero's} threshold to be .33 instead of the .5 suggested in \citet{Latona2024TheAR} increases the recall dramatically and raises the $F_{1}$ to 0.84. }\label{table:metrics}
\end{table}

\subsection{Comparing detection tools}
\label{sec:comp}

Before evaluating at scale, we aim to the compare performance of the three models described in Section~\ref{sec:tools}. We randomly sample the United Nations press releases published between 2020 and 2021---substantially prior to the release of ChatGPT---for a collection of 50 human-authored texts averaging 420 words each. We then create corresponding press releases by a leading model, GPT-4o~\citep{openai2024gpt4}.\footnote{While \citet{wang-etal-2024-m4} note that different models may be detected differently, this is arguably the model most likely to be used by somebody with a non-technical background.  Our prompting methodology is provided the in Appendix.}   The tools studied are designed and tested primarily with English sources, so we limit the scope of our experiments to English (Limitations).  
 
We also create versions of the UN press release dataset that contain texts with ratios of 1/3rd or 2/3rd AI/human content to determine how well the detectors can identify proportions of AI content embedded within human-authored texts. Detection in this situation has particular relevance for education, since students may start an essay but employ AI to lengthen or modify its content~\citep{fuchs2023exploring}. 
%
This is clearly a more difficult task than the binary classification of fully-AI or fully-human.\footnote{An author without extensive knowledge of the United Nations or GenAI was tasked with classifying a mix of texts including half randomly sampled from actual press releases and half from a stratified random sample of AI-generated texts (comprising $1/3$, $2/3$, and fully generated content). The author achieved a classification accuracy of only 60\%, (12\% false positive rate and 28\% false negative rate), with consistent performance across different AI mixtures.}



All three AI detectors distinguish human content from AI-generated and hybrid content. 
%
Yet on this data set, in contrast with prior work, we find that \texttt{GPTZero} substantially outperforms \texttt{Binoculars} and \texttt{Ghostbuster} with AUROC scores of 0.98 for \texttt{GPTZero}, compared with 0.85, and 0.81 for \texttt{Ghostbuster}, and \texttt{Binoculars} (Table~\ref{table:metrics}).

\begin{comment}
\begin{table}
  \centering
  \begin{tabular}{ll}
    \hline
    \textbf{Tool}  & \textbf{Type}  \\
    \hline
    GPTZero & Black Box \\
    Binoculars & Open Source \\ 
    Ghostbuster & Open Source \\
  \end{tabular}
  \caption{Tools}
  \label{tab:accents}
\end{table}
\end{comment}

We also compare rates of detection for both \texttt{GPTZero} and \texttt{Binoculars} across the period of time before high-performing LLMs became available to the public and since that time.\footnote{We do not include \texttt{Ghostbuster} in this analysis as it does not readily scale to thousands of queries.} We reason that detectors should display increased detection after the release of ChatGPT in November of 2022. %As is evident in Figure 2, 
%
We observe the expected increase approximately six months after ChatGPT's release with \texttt{GPTZero} (Figure~\ref{fig:UN}). 
%
\texttt{Binoculars} on the other hand, flags \textit{more} content than GPTZero before November of 2022 as AI and, flags \textit{less} content as AI than GPTZero 2023 onwards.
%
%By default, \texttt{Binoculars} classifies perplexity ratios below a threshold of .901 as generated by AI, as displayed in the bottom panel of Figure 2.
    
To summarize, the current ablation study indicates that \texttt{GPTZero} has higher accuracy when detecting both mixed and fully AI-generated content than \texttt{Binoculars} or \texttt{Ghostbuster}. 
%
Our observation of detection rates across time also indicates that \texttt{GPTZero} is more accurate than \texttt{Binoculars}, since only \texttt{GPTZero} shows an increase in AI content between 2022-2024, while \texttt{Binoculars} indicates a steady rate of flagged texted across time. %$\textbf{(does it ? there are more blue dots to the right than the left; is that not meaningful?)}

\subsection{Exploring detected content}

Press releases that are detected as primarily AI deal can be societal (Figure~\ref{fig:albania}), emotional (Figure~\ref{fig:belize}), and procedural (Figure~\ref{fig:bangladesh}).
%
The marked increase in UN press releases flagged as AI may stem from translations into English, although the authors are often educated in English-speaking countries.  

%EXAMPLE WHERE THEY AGREE
%EXAMPLES WHERE THEY DISAGREE


\begin{figure}[t]
\centering
\includegraphics[width=.9\linewidth]{figures/fig2.png} 
  \caption {According to \texttt{GPTZero}, some new Wikipedia pages and press releases by United Nations country teams are likely to be predominantly generated by AI.
  However, news articles and contentious Reddit threads contain little AI generated content. }
  \label{fig:totals}
  
\end{figure}

\begin{comment}
\begin{table}
  \centering
  \begin{tabular}{lll}
    \hline
    \textbf{Source}  & \textbf{\# of Articles} &  \textbf{Ratio} \\
    \hline
    UN Press & 8326 & 10.0\% \\
    News & 50 & 0.0\% \\
    Wikipedia & 6705 & 6.0\% \\
    Reddit & 4747 & 0.5\% \\         
  \end{tabular}
  \caption{Data and AI detection according to \texttt{GPTZero}}
  \label{tab:accents}
\end{table}
\end{comment}



%In order to compare the rates at which three leading AI detectors---Ghostbuster~\citep{verma2023ghostbuster}, \texttt{Binoculars}~\citep{hans2024spotting}, \texttt{GPTZero}---indicate machine-generated content across the period of time before and after LLMs became widely available. 
%


%
%Furthermore, this distinction proves challenging for a human.

%
    
